Generative Visual Dialogue System via Adaptive Reasoning and Weighted Likelihood Estimation

The key challenge of generative Visual Dialogue (VD) systems is to respond to human queries with informative answers in natural and contiguous conversation flow. Traditional Maximum Likelihood Estimation (MLE)-based methods only learn from positive responses but ignore the negative responses, and consequently tend to yield safe or generic responses. To address this issue, we propose a novel training scheme in conjunction with weighted likelihood estimation (WLE) method. Furthermore, an adaptive multi-modal reasoning module is designed, to accommodate various dialogue scenarios automatically and select relevant information accordingly. The experimental results on the VisDial benchmark demonstrate the superiority of our proposed algorithm over other state-of-the-art approaches, with an improvement of 5.81% on recall@10.

==> IJCAI 2019 camera ready/fig_att_viz.tex <==
\begin{figure}
\centering
% \includegraphics[trim=30 20 275 80, clip,width=0.7\columnwidth]{figures/att_viz.pdf}
\includegraphics[trim=0 120 600 13, clip,width=0.8\columnwidth]{figures/att_viz_adaptive.pdf}
\caption{Visualization of image attention heatmaps for different questions and reasoning steps. Regions of attention are highlighted in blue.}
\label{fig:att_viz}
\end{figure}

==> IJCAI 2019 camera ready/fig_challenge.tex <==
\begin{figure}
\centering
\includegraphics[trim=60 630 210 80, clip,width=0.8\columnwidth]{figures/challenge.pdf}
\caption{Results of the top-10 teams in the first visual dialog challenge. As the only team in top-10 uses generative visual dialogue system, we are ranked as the 6th place (highlighted with gray color). Our NDCG score is comparable with other discriminative systems.}
\label{fig:challenge}
\end{figure}

==> IJCAI 2019 camera ready/fig_demo.tex <==
\begin{figure}
\centering
\includegraphics[trim=0 0 0 0, clip,width=0.7\columnwidth]{figures/demo_compact.png}
\caption{Screenshot of the proposed generative visual dialogue system demo video, where users can input their own questions.}
\label{fig:demo}
\end{figure}

==> IJCAI 2019 camera ready/fig_example_comparison.tex <==
\begin{figure}
\centering
\addtolength{\subfigcapskip}{-0.2in}
\addtolength{\subfigbottomskip}{-0.2in}
\subfigure[]{
\label{fig:example}
\includegraphics[trim=170 130 910 280,clip,scale=0.3]{figures/comparison.pdf}}
\subfigure[]{
\label{fig:comparison}
\includegraphics[trim=520 130 490 280,clip,scale=0.3]{figures/comparison.pdf}}
\vspace{-0.05in}
\caption{(a) An example from the VisDial dataset, and (b) comparison
between MLE, GAN and WLE, where positive responses are highlighted in
blue.  The MLE-based generator learn from data in positive answers only.
The GAN-based generator learn from data in negative answers through
discriminators indirectly.  Our WLE-based generator learn from data in
both positive and negative answers.}
\end{figure}

==> IJCAI 2019 camera ready/fig_qualitative.tex <==
\begin{figure*}
\centering
%\includegraphics[trim=70 110 340 60,clip,width=0.7\textwidth]{figures/qualitative.pdf}
\includegraphics[trim=70 274 340 60,clip,width=0.9\textwidth]{figures/qualitative_compact.pdf}
\caption{Qualitative results on \texttt{test}. The questions and answers are truncated at 16 and 8, respectively, same as our data pre-processing. }
\label{fig:qualitative}
\end{figure*}

==> IJCAI 2019 camera ready/fig_rank_example.tex <==
\begin{figure}
\centering
%\includegraphics[trim=100 288 160 90,clip,width=0.8\textwidth]{figures/top-10_example.pdf}
%\includegraphics[trim=100 288 160 270,clip,width=0.75\textwidth]{figures/top-10_example.pdf}
\includegraphics[trim=100 498 555 71,clip,width=0.9\columnwidth]{figures/top-10_example_compact.pdf}
\caption{Examples of top-10 responses ranked by our model. When there are multiple correct responses to the question, our model may choose other candidates that are semantically similar to the human response. The human responses are highlighted in blue.}
\label{fig:rank_example}
\end{figure}

==> IJCAI 2019 camera ready/fig_recurrent_attention.tex <==
\begin{figure}
\centering
\includegraphics[trim=360 210 430 100,clip,width=0.75\columnwidth]{figures/recurrent_attention.pdf}
\caption{The adaptive multi-modal reasoning.}
\label{fig:recurrent_attention}
\end{figure}

==> IJCAI 2019 camera ready/tb_ablation_results.tex <==
\begin{table}
\centering
\tabcolsep=0.11cm
\singlespace
\scalebox{0.9}{
\begin{tabulary}{2\columnwidth}{LCCCCCC}
\toprule
Model & MRR & R@1 & R@5 & R@10 & Mean\\
\midrule
\small HCIAE-MLE
&0.5386 			&44.06 		&63.55 		&69.24 		& 16.01		\\
\small HCIAE-GAN
&0.5467			&44.35		&65.28		&71.55 		& 14.23\\
%\midrule
\small HCIAE-WLE	
&0.5494 			&43.43		&66.88		&75.59		&9.93\\
\small AMR-MLE		
&0.5403 			&44.17		&63.86		&69.67		&15.49\\
\small AMR-WLE		
&\tbf{0.5614}	&\tbf{44.49}	&\tbf{68.75}	&\tbf{77.55}	&\tbf{9.15}\\
\midrule
\midrule
Model & $\Delta$MRR & $\Delta$R@1 & $\Delta$R@5 & $\Delta$R@10 & $\Delta$Mean\\
\midrule
\small HCIAE-MLE
& ---			&---			&---			&---			&--- \\
\small HCIAE-GAN
&+0.0081 		&+0.29 		&+1.73		&+2.31		&-1.78\\
%\midrule
\small HCIAE-WLE
&+0.0108 		&-0.92 		&+3.33 		&+6.35 		&-6.08\\
\small AMR-MLE
& --- 			&---			&---			&--- 		&---\\
\small AMR-WLE
&\tbf{+0.0211}	&\tbf{+0.32}	&\tbf{+4.89}	&\tbf{+7.88}	&\tbf{-6.34}\\
\bottomrule
\end{tabulary}}
\vspace{-0.05in}
\caption{Ablation study on VisDial 0.9. Top: absolute values. Bottom: improvement from MLE models.
%The absolute values are listed on the top and the improvement from MLE models are at the bottom. 
}\label{tb:ablation_results}
\end{table}

==> IJCAI 2019 camera ready/tb_challenge.tex <==
\begin{table}
\centering
\singlespacing
\tabcolsep=0.11cm
\scalebox{0.9}{
\begin{tabulary}{\columnwidth}{LCC}
\toprule
Position & NDCG & MRR\\
\midrule
1 & 57.75 & 64.54 \\
2 & 56.45 & 62.82 \\
3 & 55.38 & 65.01 \\
4 & 55.33 & 64.68 \\
5 & 54.31 & 68.14 \\
\rowcolor{lightgray} 6 & 52.65 & 50.63 \\
7 & 50.27 & 59.73 \\
8 & 48.76 & 60.06 \\
9 & 47.79 & 62.55 \\
10 & 45.78 & 60.20 \\
\bottomrule
\end{tabulary}}
\vspace{-0.05in}
\caption{Results of the top-10 teams in the first visual dialog challenge. As the only team in top-10 uses generative visual dialogue system, we are ranked as the 6th place (highlighted with gray color). Our NDCG score is comparable with other discriminative systems.}
\label{tb:challenge}
\end{table}

==> IJCAI 2019 camera ready/tb_results.tex <==
\begin{table}
\centering
\singlespacing
\tabcolsep=0.11cm
\scalebox{0.9}{
\begin{tabulary}{\columnwidth}{LCCCCC}
\toprule
Model & MRR & R@1 & R@5 & R@10 & Mean\\
\midrule
\footnotesize LF~\scriptsize{\cite{VD}} & 0.5199	 & 41.83 & 61.78 & 67.59 & 17.07\\
\footnotesize HREA~\scriptsize{\cite{VD}} & 0.5242 & 42.28 & 62.33 & 68.17 & 16.79\\
\footnotesize MN~\scriptsize{\cite{VD}} & 0.5259 & 42.29 & 62.85 & 68.88 & 17.06\\
\footnotesize HCIAE~\scriptsize{\cite{best_of_both_worlds}} & 0.5467 & 44.35 & 65.28 & 71.55 & 14.23\\
\footnotesize FlipDial~\scriptsize{\cite{flipdial}} & 0.4549 & 34.08 & 56.18 & 61.11 & 20.38\\
\footnotesize CoAtt~\scriptsize{\cite{are_you_talking_to_me}} & 0.5578 & \textbf{46.10} & 65.69 & 71.74 & 14.43\\
%\midrule
\footnotesize Coref~\scriptsize{\cite{visual_coreference_resolution}} & 0.5350 & 43.66 & 63.54 & 69.93 & 15.69\\
\midrule
\small Ours & \textbf{0.5614} & 44.49 & \textbf{68.75} & \textbf{77.55} & \textbf{9.15}\\
\bottomrule
\end{tabulary}}
\vspace{-0.05in}
\caption{Performance of generative models on VisDial 0.9. 
`Mean' denotes mean rank, for which lower is better. 
All the models use VGG as backbone except for Coref which uses ResNet.}
\label{tb:results}
\end{table}

==> IJCAI 2019 camera ready/tb_v1.0val.tex <==
\begin{table}
\centering
\singlespacing
\tabcolsep=0.11cm
\scalebox{0.9}{
\begin{tabulary}{\columnwidth}{LCCCCC}
\toprule
Model & MRR & R@1 & R@5 & R@10 & Mean\\
\midrule
\footnotesize MN~\scriptsize{\cite{VD}} 
&0.4799      &38.18      &57.54      &64.32      &18.60\\
\footnotesize HCIAE~\scriptsize{\cite{best_of_both_worlds}} 
&0.4910      &39.35      &58.49      &64.70      &18.46\\
\footnotesize CoAtt~\scriptsize{\cite{are_you_talking_to_me}} 
&0.4925      &39.66      &58.83      &65.38      &18.15\\
\footnotesize ReDAN~\scriptsize{\cite{ReDAN}}
&0.4969      &\tbf{40.19}&59.35      &66.06      &17.92\\
\midrule
\small Ours 
&\tbf{0.5015}&38.26      &\tbf{62.54}&\tbf{72.79}&\tbf{10.71}\\
\bottomrule
\end{tabulary}}
\vspace{-0.05in}
\caption{Performance of generative models on VisDial v1.0 val. 
%`Mean' denotes mean rank, for which lower is better. 
Results of previous work are reported by ReDAN.}
\label{tb:v1_0val}
\end{table}

==> fig_demo.tex <==
\begin{figure}
\centering
\includegraphics[trim=0 0 0 0, clip,width=0.7\columnwidth]{figures/demo_compact.png}
\caption{Screenshot of the proposed generative visual dialogue system demo video, where users can input their own questions.}
\label{fig:demo}
\end{figure}

==> tb_challenge.tex <==
\begin{table}
\centering
\singlespacing
\tabcolsep=0.11cm
\scalebox{0.9}{
\begin{tabulary}{\columnwidth}{LCC}
\toprule
Position & NDCG & MRR\\
\midrule
1 & 57.75 & 64.54 \\
2 & 56.45 & 62.82 \\
3 & 55.38 & 65.01 \\
4 & 55.33 & 64.68 \\
5 & 54.31 & 68.14 \\
\rowcolor{lightgray} 6 & 52.65 & 50.63 \\
7 & 50.27 & 59.73 \\
8 & 48.76 & 60.06 \\
9 & 47.79 & 62.55 \\
10 & 45.78 & 60.20 \\
\bottomrule
\end{tabulary}}
\vspace{-0.05in}
\caption{Results of the top-10 teams in the first visual dialog challenge. As the only team in top-10 uses generative visual dialogue system, we are ranked as the 6th place (highlighted with gray color). Our NDCG score is comparable with other discriminative systems.}
\label{tb:challenge}
\end{table}
